Cepheids as distance indicators and stellar tracers

We review the phenomenology of classical Cepheids (CCs), Anomalous Cepheids (ACs) and type II Cepheids (TIICs) in the Milky Way (MW) and in the Magellanic Clouds (MCs). We also examine the Hertzsprung progression in different stellar systems by using the shape of I-band light curves (Fourier parameters) and observables based on the difference in magnitude and in phase between the bump and the minimum in luminosity. The distribution of Cepheids in optical and in optical-near infrared (NIR) color--magnitude diagrams is investigated to constrain the topology of the instability strip. The use of Cepheids as tracers of young (CCs), intermediate (ACs) and old (TIICs) stellar populations are brought forward by the comparison between observations (MCs) and cluster isochrones covering a broad range in stellar ages and in chemical compositions. The different diagnostics adopted to estimate individual distances (period--luminosity, period--Wesenheit, period--luminosity--color relations) are reviewed together with pros and cons in the use of fundamental and overtones, optical and NIR photometric bands, and reddening free pseudo magnitudes (Wesenheit). We also discuss the use of CCs as stellar tracers and the radial gradients among the different groups of elements (iron, alpha, neutron-capture) together with their age-dependence. Finally, we briefly outline the role that near-future space and ground-based facilities will play in the astrophysical and cosmological use of Cepheids.

==> tab_heburn+Idup_over_reviewstyle.tex <==
\begin{table}
\begin{center}
\caption{
Evolutionary parameters at Central He-burning ignition and at I dredge-up (IDUP) from BaSTI2 scaled-solar \citep{caffauetal2011} evolutionary models taking into account of convective core overshooting during central hydrogen burning phases.  
}
\label{He_burn+IDUP_over}
{\scriptsize
\begin{tabular}{ccccccc}
\noalign{\smallskip}\hline\hline\noalign{\smallskip}
    & \multicolumn{3}{c}{He burning}    & \multicolumn{3}{c}{IDUP}    \\ 
   M/M$_\odot$  & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%
\multicolumn{7}{c}{[Fe/H]=+0.06, Y=0.2695} \\
    \multicolumn{7}{c}{}   \\ 
%
    % 2.0   &   9.08007889 & 1.474264 & 3.701339 \\
    % 2.1   &   9.01507665 & 2.448737 & 3.637050 \\
    % 2.2   &   8.95512166 & 2.463532 & 3.639037 \\
    % 2.3   &   8.89910102 & 2.466122 & 3.641789 \\
    % 2.4   &   8.84662428 & 2.478242 & 3.643688 \\
    2.5   &   8.796 & 2.501 & 3.645 &   2.538 & 3.642  & 8.797\\
    2.6   &   8.749 & 2.523 & 3.645 &   2.567 & 3.642  & 8.749\\
    2.8   &   8.660 & 2.590 & 3.645 &   2.635 & 3.641  & 8.660\\
    3.0   &   8.578 & 2.661 & 3.644 &   2.712 & 3.640  & 8.579\\
    3.5   &   8.400 & 2.840 & 3.639 &   2.894 & 3.635  & 8.400\\
    4.0   &   8.249 & 3.013 & 3.634 &   3.071 & 3.629  & 8.250\\
    4.5   &   8.120 & 3.173 & 3.628 &   3.231 & 3.622  & 8.121\\
    5.0   &   8.004 & 3.312 & 3.622 &   3.380 & 3.616  & 8.004\\
    5.5   &   7.905 & 3.449 & 3.617 &   3.523 & 3.610  & 7.906\\
    6.0   &   7.818 & 3.576 & 3.612 &   3.649 & 3.604  & 7.818\\
    6.5   &   7.740 & 3.692 & 3.607 &   3.765 & 3.599  & 7.741\\
    7.0   &   7.670 & 3.798 & 3.602 &   3.872 & 3.595  & 7.671\\
    7.5   &   7.607 & 3.896 & 3.598 &   3.972 & 3.590  & 7.608\\
    8.0   &   7.550 & 3.987 & 3.594 &   4.064 & 3.586  & 7.551\\
    8.5   &   7.498 & 4.069 & 3.591 &   4.150 & 3.583  & 7.499\\
    9.0   &   7.451 & 4.153 & 3.587 &   4.229 & 3.579  & 7.451\\
    9.5   &   7.407 & 4.236 & 3.583 &   4.303 & 3.576  & 7.408\\
   10.0   &   7.367 & 4.312 & 3.580 &   4.372 & 3.574  & 7.367\\
   11.0   &   7.295 & 3.893 & 3.640 &   4.496 & 3.569  & 7.295\\
   12.0   &   7.234 & 4.329 & 3.942 &   4.583 & 3.568  & 7.234\\
   13.0   &   7.181 & 4.513 & 4.081 &   4.556 & 3.578  & 7.181\\
   14.0   &   7.135 & 4.653 & 4.173 &   4.787 & 3.561  & 7.177\\
   % 15.0   &   7.09023960 & 4.738234 & 4.211248 \\
    \multicolumn{7}{c}{}   \\ 
\multicolumn{7}{c}{[Fe/H]=--0.30, Y=0.2571} \\
    \multicolumn{7}{c}{}   \\ 
    % 2.0   &   8.98490728 & 2.470072 & 3.655262 \\
    % 2.1   &   8.92461751 & 2.463430 & 3.658792 \\
    % 2.2   &   8.86794334 & 2.462231 & 3.661809 \\
    % 2.3   &   8.81562425 & 2.474309 & 3.663726 \\
    % 2.4   &   8.76599189 & 2.494028 & 3.664848 \\
    2.5   &   8.718 & 2.520 & 3.665 &   2.460 & 3.670 &  8.718\\
    2.6   &   8.674 & 2.553 & 3.665 &   2.481 & 3.671 &  8.673\\
    2.8   &   8.589 & 2.621 & 3.665 &   2.540 & 3.671 &  8.589\\
    3.0   &   8.512 & 2.693 & 3.663 &   2.584 & 3.672 &  8.512\\
    3.5   &   8.344 & 2.877 & 3.659 &   2.685 & 3.674 &  8.344\\
    4.0   &   8.203 & 3.046 & 3.654 &   2.770 & 3.678 &  8.202\\
    4.5   &   8.081 & 3.206 & 3.648 &   2.878 & 3.680 &  8.081\\
    5.0   &   7.976 & 3.351 & 3.643 &   3.302 & 3.647 &  7.976\\
    5.5   &   7.879 & 3.477 & 3.639 &   3.548 & 3.632 &  7.880\\
    6.0   &   7.798 & 3.601 & 3.634 &   3.675 & 3.627 &  7.798\\
    6.5   &   7.725 & 3.716 & 3.629 &   3.788 & 3.622 &  7.725\\
    7.0   &   7.659 & 3.817 & 3.625 &   3.893 & 3.618 &  7.659\\
    7.5   &   7.600 & 3.912 & 3.621 &   3.992 & 3.614 &  7.600\\
    8.0   &   7.546 & 3.978 & 3.620 &   4.082 & 3.610 &  7.546\\
    8.5   &   7.497 & 4.082 & 3.615 &   4.168 & 3.607 &  7.498\\
    9.0   &   7.452 & 4.128 & 3.615 &   4.246 & 3.604 &  7.452\\
    9.5   &   7.410 & 3.949 & 3.638 &   4.317 & 3.601 &  7.411\\
   10.0   &   7.373 & 4.060 & 3.757 &   4.385 & 3.599 &  7.373\\
   11.0   &   7.304 & 4.281 & 3.954 &   4.496 & 3.595 &  7.304\\
   12.0   &   7.244 & 4.436 & 4.088 &   4.553 & 3.596 &  7.245\\
   13.0   &   7.192 & 4.552 & 4.175 &   4.579 & 3.601 &  7.192\\
   14.0   &   7.145 & 4.680 & 4.255 &   4.813 & 3.586 &  7.185\\
   % 15.0   &   7.10713008 & 4.768887 & 4.272048 \\
\hline\noalign{\smallskip}
\multicolumn{7}{r}{\it {\footnotesize continued on next page}} \\
\end{tabular}}
\end{center}
\end{table}
%---------------------------------------------------------------------------
%				new page 
%---------------------------------------------------------------------------
\addtocounter{table}{-1}
\begin{table}[p]
\begin{center}
\caption[]{continued.}
{\scriptsize
\begin{tabular}{ccccccc}
\noalign{\smallskip}\hline\hline\noalign{\smallskip}
    & \multicolumn{3}{c}{He burning}    & \multicolumn{3}{c}{IDUP}    \\ 
   M/M$_\odot$  & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%
    \multicolumn{7}{c}{}   \\ 
\multicolumn{7}{c}{[Fe/H]=--0.60, Y=0.2521} \\
    \multicolumn{7}{c}{}   \\ 
    % 2.0   &   8.92651738 & 2.446150 & 3.672684 \\
    % 2.1   &   8.86765588 & 2.439822 & 3.675864 \\
    % 2.2   &   8.81412121 & 2.449039 & 3.677873  \\
    % 2.3   &   8.76330705 & 2.464390 & 3.679437  \\
    % 2.4   &   8.71533205 & 2.491241 & 3.679864  \\
    2.5   &   8.670 & 2.527 & 3.680 &    2.573 & 3.677 &  8.670 \\
    2.6   &   8.626 & 2.562 & 3.679 &    2.610 & 3.676 &  8.627 \\
    2.8   &   8.545 & 2.636 & 3.679 &    2.685 & 3.675 &  8.546 \\
    3.0   &   8.471 & 2.713 & 3.677 &    2.718 & 3.677 &  8.471 \\
    3.5   &   8.309 & 2.895 & 3.673 &    2.824 & 3.678 &  8.308 \\
    4.0   &   8.173 & 3.066 & 3.668 &    2.931 & 3.680 &  8.172 \\
    4.5   &   8.056 & 3.223 & 3.663 &    3.244 & 3.662 &  8.056 \\
    5.0   &   7.954 & 3.369 & 3.658 &    3.426 & 3.654 &  7.955 \\
    5.5   &   7.862 & 3.493 & 3.655 &    3.565 & 3.649 &  7.862 \\
    6.0   &   7.783 & 3.614 & 3.650 &    3.687 & 3.644 &  7.784 \\
    6.5   &   7.713 & 3.720 & 3.647 &    3.801 & 3.640 &  7.714 \\
    7.0   &   7.650 & 3.759 & 3.649 &    3.905 & 3.635 &  7.650 \\
    7.5   &   7.593 & 3.670 & 3.666 &    4.002 & 3.632 &  7.593 \\
    8.0   &   7.541 & 3.733 & 3.681 &    4.091 & 3.628 &  7.541 \\
    8.5   &   7.493 & 3.896 & 3.722 &    4.174 & 3.625 &  7.493 \\
    9.0   &   7.450 & 4.019 & 3.797 &    4.252 & 3.622 &  7.450 \\
    9.5   &   7.409 & 4.122 & 3.878 &    4.323 & 3.620 &  7.410 \\
   10.0   &   7.372 & 4.209 & 3.954 &    4.386 & 3.618 &  7.373 \\
   % 11.0   &   7.30538749 & 4.357397 & 4.074689  \\
   % 12.0   &   7.24700827 & 4.483211 & 4.173480  \\
   % 13.0   &   7.19562903 & 4.587816 & 4.240733  \\
   % 14.0   &   7.15006586 & 4.691456 & 4.288631  \\
   % 15.0   &   7.10927467 & 4.768207 & 4.319907  \\
    \multicolumn{7}{c}{}   \\ 
\multicolumn{7}{c}{[Fe/H]=--0.90, Y=0.2496} \\
    \multicolumn{7}{c}{}   \\ 
    % 2.0   &   8.88591854 & 2.408472 & 3.687955 \\
    % 2.1   &   8.83017738 & 2.414715 & 3.689956 \\
    % 2.2   &   8.77726651 & 2.426683 & 3.691555 \\
    % 2.3   &   8.72786997 & 2.456485 & 3.691896 \\
    % 2.4   &   8.68106008 & 2.491549 & 3.691952 \\
    2.5   &   8.636 & 2.527 & 3.692 &   2.571 & 3.689 &  8.637\\
    2.6   &   8.594 & 2.563 & 3.692 &   2.611 & 3.689 &  8.594\\
    2.8   &   8.515 & 2.638 & 3.691 &   2.688 & 3.688 &  8.515\\
    3.0   &   8.443 & 2.719 & 3.689 &   2.766 & 3.686 &  8.443\\
    3.5   &   8.285 & 2.902 & 3.685 &   2.955 & 3.682 &  8.285\\
    4.0   &   8.152 & 3.075 & 3.681 &   3.126 & 3.677 &  8.153\\
    4.5   &   8.038 & 3.230 & 3.677 &   3.262 & 3.675 &  8.042\\
    5.0   &   7.940 & 3.373 & 3.673 &   3.404 & 3.670 &  7.940\\
    5.5   &   7.850 & 3.482 & 3.671 &   3.569 & 3.663 &  7.851\\
    6.0   &   7.774 & 3.482 & 3.678 &   3.690 & 3.659 &  7.774\\
    6.5   &   7.705 & 3.515 & 3.693 &   3.803 & 3.655 &  7.706\\
    7.0   &   7.644 & 3.683 & 3.717 &   3.907 & 3.651 &  7.644\\
    7.5   &   7.588 & 3.831 & 3.798 &   4.003 & 3.648 &  7.588\\
    8.0   &   7.537 & 3.943 & 3.865 &   4.090 & 3.645 &  7.537\\
    8.5   &   7.490 & 4.038 & 3.918 &   4.175 & 3.642 &  7.491\\
    9.0   &   7.447 & 4.124 & 3.965 &   4.252 & 3.640 &  7.448\\
    9.5   &   7.408 & 4.199 & 4.013 &   4.322 & 3.637 &  7.408\\
   % 10.0   &   7.37110227 & 4.268677 & 4.070103 \\
   % 11.0   &   7.30534985 & 4.397286 & 4.157821 \\
   % 12.0   &   7.24749617 & 4.506278 & 4.238860 \\
   % 13.0   &   7.19678660 & 4.605303 & 4.298623 \\
\hline\noalign{\smallskip}
\end{tabular}}
\end{center}
\end{table}


==> tab_heburn+Idup_reviewstyle.tex <==
\begin{table}
\begin{center}
\caption{
Evolutionary parameters at Central He-burning ignition and at I dredge-up (IDUP) from BaSTI2 scaled solar \citep{caffauetal2011} canonical evolutionary models.
}
\label{He_burn+IDUP}
{\scriptsize
\begin{tabular}{ccccccc}
\noalign{\smallskip}\hline\hline\noalign{\smallskip}
    & \multicolumn{3}{c}{He burning}    & \multicolumn{3}{c}{IDUP}     \\ 
   M/M$_\odot$  & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%
\multicolumn{7}{c}{[Fe/H]=+0.06, Y=0.2695} \\
    \multicolumn{7}{c}{}   \\ 
    2.5  &    8.726  &  2.353  &  3.653 &    2.268  &  3.659   &  8.724 \\ 
    2.6  &    8.676  &  2.342  &  3.656 &    2.347  &  3.656   &  8.676 \\ 
    2.8  &    8.587  &  2.365  &  3.659 &    2.400  &  3.657   &  8.587 \\ 
    3.0  &    8.505  &  2.409  &  3.661 &    2.436  &  3.659   &  8.506 \\ 
    3.5  &    8.328  &  2.562  &  3.659 &    2.534  &  3.661   &  8.330 \\ 
    4.0  &    8.177  &  2.716  &  3.655 &    2.621  &  3.663   &  8.177 \\ 
    4.5  &    8.048  &  2.863  &  3.651 &    2.691  &  3.666   &  8.047 \\ 
    5.0  &    7.931  &  3.000  &  3.646 &    3.064  &  3.641   &  7.931 \\ 
    5.5  &    7.833  &  3.129  &  3.642 &    3.194  &  3.636   &  7.833 \\ 
    6.0  &    7.745  &  3.249  &  3.637 &    3.320  &  3.631   &  7.745 \\ 
    6.5  &    7.667  &  3.364  &  3.633 &    3.437  &  3.626   &  7.668 \\ 
    7.0  &    7.598  &  3.473  &  3.628 &    3.549  &  3.621   &  7.598 \\ 
    7.5  &    7.536  &  3.568  &  3.625 &    3.655  &  3.617   &  7.536 \\ 
    8.0  &    7.479  &  3.601  &  3.627 &    3.755  &  3.612   &  7.480 \\ 
    8.5  &    7.428  &  3.493  &  3.642 &    3.848  &  3.608   &  7.429 \\ 
    9.0  &    7.381  &  3.449  &  3.665 &    3.937  &  3.604   &  7.382 \\ 
    9.5  &    7.338  &  3.702  &  3.767 &    4.011  &  3.601   &  7.339 \\ 
   10.0  &    7.299  &  3.900  &  3.913 &    4.057  &  3.600   &  7.300 \\ 
   11.0  &    7.229  &  4.139  &  4.091 &    4.070  &  3.605   &  7.230 \\ 
   12.0  &    7.189  &  4.324  &  4.210 &    4.328  &  3.596   &  7.257 \\ 
   13.0  &    7.147  &  4.447  &  4.238 &    4.537  &  3.577   &  7.216 \\ 
   14.0  &    7.140  &  4.558  &  4.279 &    4.715  &  3.564   &  7.197 \\ 
    \multicolumn{7}{c}{}   \\ 
\multicolumn{7}{c}{[Fe/H]=--0.30, Y=0.2571} \\
    \multicolumn{7}{c}{}   \\ 
%====================================================================================
%   M/Msun      logt       logL      logTe              
%%====================================================================================
    2.5  &    8.647  &  2.330  &  3.676 &    2.358  &  3.674   &  8.648 \\
    2.6  &    8.602  &  2.332  &  3.678 &    2.370  &  3.676   &  8.602 \\
    2.8  &    8.517  &  2.367  &  3.680 &    2.412  &  3.677   &  8.518 \\
    3.0  &    8.440  &  2.419  &  3.681 &    2.468  &  3.678   &  8.440 \\
    3.5  &    8.271  &  2.579  &  3.679 &    2.632  &  3.675   &  8.271 \\
    4.0  &    8.130  &  2.731  &  3.676 &    2.735  &  3.676   &  8.130 \\
    4.5  &    8.008  &  2.880  &  3.671 &    2.826  &  3.676   &  8.008 \\
    5.0  &    7.903  &  3.017  &  3.668 &    3.078  &  3.663   &  7.902 \\
    5.5  &    7.806  &  3.133  &  3.665 &    3.211  &  3.658   &  7.806 \\
    6.0  &    7.724  &  3.193  &  3.666 &    3.338  &  3.653   &  7.725 \\
    6.5  &    7.651  &  3.139  &  3.681 &    3.456  &  3.648   &  7.652 \\
    7.0  &    7.586  &  3.236  &  3.698 &    3.570  &  3.644   &  7.587 \\
    7.5  &    7.528  &  3.431  &  3.729 &    3.673  &  3.639   &  7.528 \\
    8.0  &    7.475  &  3.592  &  3.801 &    3.773  &  3.633   &  7.476 \\
    8.5  &    7.427  &  3.728  &  3.879 &    3.862  &  3.631   &  7.427 \\
    9.0  &    7.383  &  3.850  &  3.950 &    3.940  &  3.628   &  7.383 \\
    9.5  &    7.343  &  3.981  &  4.040 &    3.974  &  3.629   &  7.343 \\
   10.0  &    7.306  &  4.068  &  4.104 &    3.976  &  3.633   &  7.307 \\
   11.0  &    7.239  &  4.243  &  4.208 &    4.364  &  3.608   &  7.307 \\
   12.0  &    7.200  &  4.362  &  4.268 &    4.445  &  3.607   &  7.266 \\
\hline\noalign{\smallskip}
\multicolumn{7}{r}{\it {\footnotesize continued on next page}} \\
\end{tabular}}
\end{center}
\end{table}
%---------------------------------------------------------------------------
%				new page 
%---------------------------------------------------------------------------
\addtocounter{table}{-1}
\begin{table}[p]
\begin{center}
\caption[]{continued.}
{\scriptsize
\begin{tabular}{ccccccc}
\noalign{\smallskip}\hline\hline\noalign{\smallskip}
    & \multicolumn{3}{c}{He burning}    & \multicolumn{3}{c}{IDUP}     \\ 
   M/M$_\odot$  & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%
    \multicolumn{7}{c}{}   \\ 
\multicolumn{7}{c}{[Fe/H]=--0.60, Y=0.2521} \\
    \multicolumn{7}{c}{}   \\ 
%======================================================
%   M/Msun      logt       logL      logTe              
%======================================================
    2.5  &      8.598  &  2.296  &  3.692 &   2.341  & 3.690   & 8.599 \\
    2.6  &      8.554  &  2.309  &  3.694 &   2.330  & 3.693   & 8.554 \\
    2.8  &      8.472  &  2.355  &  3.695 &   2.404  & 3.692   & 8.473 \\
    3.0  &      8.398  &  2.418  &  3.695 &   2.466  & 3.692   & 8.398 \\
    3.5  &      8.236  &  2.581  &  3.693 &   2.633  & 3.689   & 8.236 \\
    4.0  &      8.099  &  2.737  &  3.690 &   2.795  & 3.686   & 8.100 \\
    4.5  &      7.982  &  2.878  &  3.687 &   2.944  & 3.682   & 7.983 \\
    5.0  &      7.880  &  2.917  &  3.692 &   3.057  & 3.681   & 7.885 \\
    5.5  &      7.788  &  2.960  &  3.714 &   3.225  & 3.673   & 7.789 \\
    6.0  &      7.709  &  3.196  &  3.756 &   3.351  & 3.668   & 7.710 \\
    6.5  &      7.640  &  3.381  &  3.837 &   3.468  & 3.664   & 7.640 \\
    7.0  &      7.577  &  3.530  &  3.894 &   3.582  & 3.660   & 7.578 \\
    7.5  &      7.521  &  3.656  &  3.939 &   3.688  & 3.656   & 7.522 \\
    8.0  &      7.470  &  3.764  &  3.986 &   3.782  & 3.652   & 7.470 \\
    8.5  &      7.423  &  3.866  &  4.031 &   3.866  & 3.648   & 7.424 \\
    9.0  &      7.381  &  3.964  &  4.088 &   3.913  & 3.648   & 7.382 \\
    9.5  &      7.342  &  4.056  &  4.149 &   4.183  & 3.634   & 7.409 \\
   10.0  &      7.306  &  4.130  &  4.186 &   4.256  & 3.631   & 7.373 \\
    \multicolumn{7}{c}{}   \\ 
\multicolumn{7}{c}{[Fe/H]=--0.90, Y=0.2496} \\
    \multicolumn{7}{c}{}   \\ 
    2.5  &      8.564  &  2.255  &  3.706 &   2.302 &3.703  &8.565 \\
    2.6  &      8.521  &  2.277  &  3.706 &   2.326 &3.704  &8.522 \\
    2.8  &      8.442  &  2.336  &  3.707 &   2.386 &3.704  &8.442 \\
    3.0  &      8.369  &  2.404  &  3.706 &   2.454 &3.703  &8.370 \\
    3.5  &      8.212  &  2.574  &  3.705 &   2.627 &3.701  &8.212 \\
    4.0  &      8.079  &  2.686  &  3.706 &   2.795 &3.698  &8.079 \\
    4.5  &      7.964  &  2.747  &  3.726 &   2.944 &3.694  &7.965 \\
    5.0  &      7.866  &  3.020  &  3.783 &   3.096 &3.690  &7.867 \\
    5.5  &      7.776  &  3.227  &  3.880 &   3.231 &3.686  &7.777 \\
    6.0  &      7.700  &  3.387  &  3.939 &   3.358 &3.682  &7.701 \\
    6.5  &      7.632  &  3.523  &  3.983 &   3.477 &3.678  &7.633 \\
    7.0  &      7.571  &  3.643  &  4.021 &   3.587 &3.675  &7.572 \\
    7.5  &      7.516  &  3.750  &  4.051 &   3.691 &3.671  &7.518 \\
    8.0  &      7.467  &  3.843  &  4.081 &   3.784 &3.667  &7.468 \\
    8.5  &      7.421  &  3.929  &  4.120 &   3.848 &3.666  &7.423 \\
    9.0  &      7.379  &  4.016  &  4.176 &   4.289 &3.635  &7.447 \\
    9.5  &      7.341  &  4.095  &  4.206 &   4.375 &3.631  &7.407 \\
\hline\noalign{\smallskip}
\end{tabular}}
\end{center}
\end{table}


==> tab_heburn_over_reviewstyle.tex <==
\begin{table}
\begin{center}
\caption{
Evolutionary parameters at central He-burning ignition from BaSTI2 scaled-solar \citep{caffauetal2011} evolutionary models taking into account convective core overshooting during central hydrogen burning phases.  
}
\label{He_burn_over}
{\scriptsize
\begin{tabular}{cccc}
\noalign{\smallskip}\hline\hline\noalign{\smallskip}
   M/M$_\odot$  & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%
\multicolumn{4}{c}{[Fe/H]=+0.06, Y=0.2695} \\
    &     &    &   \\ 
%
    % 2.0   &   9.08007889 & 1.474264 & 3.701339 \\
    % 2.1   &   9.01507665 & 2.448737 & 3.637050 \\
    % 2.2   &   8.95512166 & 2.463532 & 3.639037 \\
    % 2.3   &   8.89910102 & 2.466122 & 3.641789 \\
    % 2.4   &   8.84662428 & 2.478242 & 3.643688 \\
    2.5   &   8.796 & 2.501 & 3.645 \\
    2.6   &   8.749 & 2.523 & 3.645 \\
    2.8   &   8.660 & 2.590 & 3.645 \\
    3.0   &   8.578 & 2.661 & 3.644 \\
    3.5   &   8.400 & 2.840 & 3.639 \\
    4.0   &   8.249 & 3.013 & 3.634 \\
    4.5   &   8.120 & 3.173 & 3.628 \\
    5.0   &   8.004 & 3.312 & 3.622 \\
    5.5   &   7.905 & 3.449 & 3.617 \\
    6.0   &   7.818 & 3.576 & 3.612 \\
    6.5   &   7.740 & 3.692 & 3.607 \\
    7.0   &   7.670 & 3.798 & 3.602 \\
    7.5   &   7.607 & 3.896 & 3.598 \\
    8.0   &   7.550 & 3.987 & 3.594 \\
    8.5   &   7.498 & 4.069 & 3.591 \\
    9.0   &   7.451 & 4.153 & 3.587 \\
    9.5   &   7.407 & 4.236 & 3.583 \\
   10.0   &   7.367 & 4.312 & 3.580 \\
   11.0   &   7.295 & 3.893 & 3.640 \\
   12.0   &   7.234 & 4.329 & 3.942 \\
   13.0   &   7.181 & 4.513 & 4.081 \\
   14.0   &   7.135 & 4.653 & 4.173 \\
   % 15.0   &   7.09023960 & 4.738234 & 4.211248 \\
    &    &    &   \\ 
\multicolumn{4}{c}{[Fe/H]=--0.30, Y=0.2571} \\
    &    &    &   \\ 
    % 2.0   &   8.98490728 & 2.470072 & 3.655262 \\
    % 2.1   &   8.92461751 & 2.463430 & 3.658792 \\
    % 2.2   &   8.86794334 & 2.462231 & 3.661809 \\
    % 2.3   &   8.81562425 & 2.474309 & 3.663726 \\
    % 2.4   &   8.76599189 & 2.494028 & 3.664848 \\
    2.5   &   8.718 & 2.520 & 3.665 \\
    2.6   &   8.674 & 2.553 & 3.665 \\
    2.8   &   8.589 & 2.621 & 3.665 \\
    3.0   &   8.512 & 2.693 & 3.663 \\
    3.5   &   8.344 & 2.877 & 3.659 \\
    4.0   &   8.203 & 3.046 & 3.654 \\
    4.5   &   8.081 & 3.206 & 3.648 \\
    5.0   &   7.976 & 3.351 & 3.643 \\
    5.5   &   7.879 & 3.477 & 3.639 \\
    6.0   &   7.798 & 3.601 & 3.634 \\
    6.5   &   7.725 & 3.716 & 3.629 \\
    7.0   &   7.659 & 3.817 & 3.625 \\
    7.5   &   7.600 & 3.912 & 3.621 \\
    8.0   &   7.546 & 3.978 & 3.620 \\
    8.5   &   7.497 & 4.082 & 3.615 \\
    9.0   &   7.452 & 4.128 & 3.615 \\
    9.5   &   7.410 & 3.949 & 3.638 \\
   10.0   &   7.373 & 4.060 & 3.757 \\
   11.0   &   7.304 & 4.281 & 3.954 \\
   12.0   &   7.244 & 4.436 & 4.088 \\
   13.0   &   7.192 & 4.552 & 4.175 \\
   14.0   &   7.145 & 4.680 & 4.255 \\
   % 15.0   &   7.10713008 & 4.768887 & 4.272048 \\
\hline\noalign{\smallskip}
\multicolumn{4}{r}{\it {\footnotesize continued on next page}} \\
\end{tabular}}
\end{center}
\end{table}
%---------------------------------------------------------------------------
%				new page 
%---------------------------------------------------------------------------
\addtocounter{table}{-1}
\begin{table}[p]
\begin{center}
\caption[]{continued.}
{\scriptsize
\begin{tabular}{cccc}
\noalign{\smallskip}\hline\hline\noalign{\smallskip}
   M/M$_\odot$  & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%
    &     &    &   \\ 
\multicolumn{4}{c}{[Fe/H]=--0.60, Y=0.2521} \\
    &     &    &   \\ 
    % 2.0   &   8.92651738 & 2.446150 & 3.672684 \\
    % 2.1   &   8.86765588 & 2.439822 & 3.675864 \\
    % 2.2   &   8.81412121 & 2.449039 & 3.677873  \\
    % 2.3   &   8.76330705 & 2.464390 & 3.679437  \\
    % 2.4   &   8.71533205 & 2.491241 & 3.679864  \\
    2.5   &   8.670 & 2.527 & 3.680  \\
    2.6   &   8.626 & 2.562 & 3.679  \\
    2.8   &   8.545 & 2.636 & 3.679  \\
    3.0   &   8.471 & 2.713 & 3.677  \\
    3.5   &   8.309 & 2.895 & 3.673  \\
    4.0   &   8.173 & 3.066 & 3.668  \\
    4.5   &   8.056 & 3.223 & 3.663  \\
    5.0   &   7.954 & 3.369 & 3.658  \\
    5.5   &   7.862 & 3.493 & 3.655  \\
    6.0   &   7.783 & 3.614 & 3.650  \\
    6.5   &   7.713 & 3.720 & 3.647  \\
    7.0   &   7.650 & 3.759 & 3.649  \\
    7.5   &   7.593 & 3.670 & 3.666  \\
    8.0   &   7.541 & 3.733 & 3.681  \\
    8.5   &   7.493 & 3.896 & 3.722  \\
    9.0   &   7.450 & 4.019 & 3.797  \\
    9.5   &   7.409 & 4.122 & 3.878  \\
   10.0   &   7.372 & 4.209 & 3.954  \\
   % 11.0   &   7.30538749 & 4.357397 & 4.074689  \\
   % 12.0   &   7.24700827 & 4.483211 & 4.173480  \\
   % 13.0   &   7.19562903 & 4.587816 & 4.240733  \\
   % 14.0   &   7.15006586 & 4.691456 & 4.288631  \\
   % 15.0   &   7.10927467 & 4.768207 & 4.319907  \\
    &     &    &   \\ 
\multicolumn{4}{c}{[Fe/H]=--0.90, Y=0.2496} \\
    &     &    &   \\ 
    % 2.0   &   8.88591854 & 2.408472 & 3.687955 \\
    % 2.1   &   8.83017738 & 2.414715 & 3.689956 \\
    % 2.2   &   8.77726651 & 2.426683 & 3.691555 \\
    % 2.3   &   8.72786997 & 2.456485 & 3.691896 \\
    % 2.4   &   8.68106008 & 2.491549 & 3.691952 \\
    2.5   &   8.636 & 2.527 & 3.692 \\
    2.6   &   8.594 & 2.563 & 3.692 \\
    2.8   &   8.515 & 2.638 & 3.691 \\
    3.0   &   8.443 & 2.719 & 3.689 \\
    3.5   &   8.285 & 2.902 & 3.685 \\
    4.0   &   8.152 & 3.075 & 3.681 \\
    4.5   &   8.038 & 3.230 & 3.677 \\
    5.0   &   7.940 & 3.373 & 3.673 \\
    5.5   &   7.850 & 3.482 & 3.671 \\
    6.0   &   7.774 & 3.482 & 3.678 \\
    6.5   &   7.705 & 3.515 & 3.693 \\
    7.0   &   7.644 & 3.683 & 3.717 \\
    7.5   &   7.588 & 3.831 & 3.798 \\
    8.0   &   7.537 & 3.943 & 3.865 \\
    8.5   &   7.490 & 4.038 & 3.918 \\
    9.0   &   7.447 & 4.124 & 3.965 \\
    9.5   &   7.408 & 4.199 & 4.013 \\
   % 10.0   &   7.37110227 & 4.268677 & 4.070103 \\
   % 11.0   &   7.30534985 & 4.397286 & 4.157821 \\
   % 12.0   &   7.24749617 & 4.506278 & 4.238860 \\
   % 13.0   &   7.19678660 & 4.605303 & 4.298623 \\
\hline\noalign{\smallskip}
\end{tabular}}
\end{center}
\end{table}


==> tab_heburn_reviewstyle.tex <==
\begin{table}
\begin{center}
\caption{
Evolutionary parameters at central He-burning ignition from BaSTI2 scaled solar \citep{caffauetal2011} canonical evolutionary models.
}
\label{He_burn}
{\scriptsize
\begin{tabular}{cccc}
\noalign{\smallskip}\hline\hline\noalign{\smallskip}
   M/M$_\odot$  & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%
\multicolumn{4}{c}{[Fe/H]=+0.06, Y=0.2695} \\
    &     &    &   \\ 
    2.5  &    8.726  &  2.353  &  3.653  \\ 
    2.6  &    8.676  &  2.342  &  3.656  \\ 
    2.8  &    8.587  &  2.365  &  3.659  \\ 
    3.0  &    8.505  &  2.409  &  3.661  \\ 
    3.5  &    8.328  &  2.562  &  3.659  \\ 
    4.0  &    8.177  &  2.716  &  3.655  \\ 
    4.5  &    8.048  &  2.863  &  3.651  \\ 
    5.0  &    7.931  &  3.000  &  3.646  \\ 
    5.5  &    7.833  &  3.129  &  3.642  \\ 
    6.0  &    7.745  &  3.249  &  3.637  \\ 
    6.5  &    7.667  &  3.364  &  3.633  \\ 
    7.0  &    7.598  &  3.473  &  3.628  \\ 
    7.5  &    7.536  &  3.568  &  3.625  \\ 
    8.0  &    7.479  &  3.601  &  3.627  \\ 
    8.5  &    7.428  &  3.493  &  3.642  \\ 
    9.0  &    7.381  &  3.449  &  3.665  \\ 
    9.5  &    7.338  &  3.702  &  3.767  \\ 
   10.0  &    7.299  &  3.900  &  3.913  \\ 
   11.0  &    7.229  &  4.139  &  4.091  \\ 
   12.0  &    7.189  &  4.324  &  4.210  \\ 
   13.0  &    7.147  &  4.447  &  4.238  \\ 
   14.0  &    7.140  &  4.558  &  4.279  \\ 
    &    &    &   \\ 
\multicolumn{4}{c}{[Fe/H]=--0.30, Y=0.2571} \\
    &    &    &   \\ 
%====================================================================================
%   M/Msun      logt       logL      logTe              
%%====================================================================================
    2.5  &    8.647  &  2.330  &  3.676  \\
    2.6  &    8.602  &  2.332  &  3.678  \\
    2.8  &    8.517  &  2.367  &  3.680  \\
    3.0  &    8.440  &  2.419  &  3.681  \\
    3.5  &    8.271  &  2.579  &  3.679  \\
    4.0  &    8.130  &  2.731  &  3.676  \\
    4.5  &    8.008  &  2.880  &  3.671  \\
    5.0  &    7.903  &  3.017  &  3.668  \\
    5.5  &    7.806  &  3.133  &  3.665  \\
    6.0  &    7.724  &  3.193  &  3.666  \\
    6.5  &    7.651  &  3.139  &  3.681  \\
    7.0  &    7.586  &  3.236  &  3.698  \\
    7.5  &    7.528  &  3.431  &  3.729  \\
    8.0  &    7.475  &  3.592  &  3.801  \\
    8.5  &    7.427  &  3.728  &  3.879  \\
    9.0  &    7.383  &  3.850  &  3.950  \\
    9.5  &    7.343  &  3.981  &  4.040  \\
   10.0  &    7.306  &  4.068  &  4.104  \\
   11.0  &    7.239  &  4.243  &  4.208  \\
   12.0  &    7.200  &  4.362  &  4.268  \\
\hline\noalign{\smallskip}
\multicolumn{4}{r}{\it {\footnotesize continued on next page}} \\
\end{tabular}}
\end{center}
\end{table}
%---------------------------------------------------------------------------
%				new page 
%---------------------------------------------------------------------------
\addtocounter{table}{-1}
\begin{table}[p]
\begin{center}
\caption[]{continued.}
{\scriptsize
\begin{tabular}{cccc}
\noalign{\smallskip}\hline\hline\noalign{\smallskip}
   M/M$_\odot$  & $\log\,t$ & $\log\,L/L_\odot$  &  $\log\,T_{eff}$ \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%
    &     &    &   \\ 
\multicolumn{4}{c}{[Fe/H]=--0.60, Y=0.2521} \\
    &     &    &   \\ 
%======================================================
%   M/Msun      logt       logL      logTe              
%======================================================
    2.5  &      8.598  &  2.296  &  3.692  \\
    2.6  &      8.554  &  2.309  &  3.694  \\
    2.8  &      8.472  &  2.355  &  3.695  \\
    3.0  &      8.398  &  2.418  &  3.695  \\
    3.5  &      8.236  &  2.581  &  3.693  \\
    4.0  &      8.099  &  2.737  &  3.690  \\
    4.5  &      7.982  &  2.878  &  3.687  \\
    5.0  &      7.880  &  2.917  &  3.692  \\
    5.5  &      7.788  &  2.960  &  3.714  \\
    6.0  &      7.709  &  3.196  &  3.756  \\
    6.5  &      7.640  &  3.381  &  3.837  \\
    7.0  &      7.577  &  3.530  &  3.894  \\
    7.5  &      7.521  &  3.656  &  3.939  \\
    8.0  &      7.470  &  3.764  &  3.986  \\
    8.5  &      7.423  &  3.866  &  4.031  \\
    9.0  &      7.381  &  3.964  &  4.088  \\
    9.5  &      7.342  &  4.056  &  4.149  \\
   10.0  &      7.306  &  4.130  &  4.186  \\
    &     &    &   \\ 
\multicolumn{4}{c}{[Fe/H]=--0.90, Y=0.2496} \\
    &     &    &   \\ 
    2.5  &      8.564  &  2.255  &  3.706  \\
    2.6  &      8.521  &  2.277  &  3.706  \\
    2.8  &      8.442  &  2.336  &  3.707  \\
    3.0  &      8.369  &  2.404  &  3.706  \\
    3.5  &      8.212  &  2.574  &  3.705  \\
    4.0  &      8.079  &  2.686  &  3.706  \\
    4.5  &      7.964  &  2.747  &  3.726  \\
    5.0  &      7.866  &  3.020  &  3.783  \\
    5.5  &      7.776  &  3.227  &  3.880  \\
    6.0  &      7.700  &  3.387  &  3.939  \\
    6.5  &      7.632  &  3.523  &  3.983  \\
    7.0  &      7.571  &  3.643  &  4.021  \\
    7.5  &      7.516  &  3.750  &  4.051  \\
    8.0  &      7.467  &  3.843  &  4.081  \\
    8.5  &      7.421  &  3.929  &  4.120  \\
    9.0  &      7.379  &  4.016  &  4.176  \\
    9.5  &      7.341  &  4.095  &  4.206  \\
\hline\noalign{\smallskip}
\end{tabular}}
\end{center}
\end{table}

